Tunable Causal Consistency: Specification and Implementation

To achieve high availability and low latency, distributed data stores often geographically replicate data at multiple sites called replicas. However, this introduces the data consistency problem. Due to the fundamental tradeoffs among consistency, availability, and latency in the presence of network partition, no a one-size-fits-all consistency model exists. To meet the needs of different applications, many popular data stores provide tunable consistency, allowing clients to specify the consistency level per individual operation. In this paper, we propose tunable causal consistency (TCC). It allows clients to choose the desired session guarantee for each operation, from the well-known four session guarantees, i.e., read your writes, monotonic reads, monotonic writes, and writes follow reads. Specifically, we first propose a formal specification of TCC in an extended (vis,ar) framework originally proposed by Burckhardt et al. Then we design a TCC protocol and develop a prototype distributed key-value store called TCCSTORE. We evaluate TCCSTORE on Aliyun. The latency is less than 38ms for all workloads and the throughput is up to about 2800 operations per second. We also show that TCC achieves better performance than causal consistency and requires a negligible overhead when compared with eventual consistency.

==> algs/cure-client-single-cvc.tex <==
% cure-client.tex

\begin{algorithm}
  \caption{Client operations at client $c$}
  \label{alg:client}
  \begin{algorithmic}[1]
    \Statex \red{$\hwvc$: Highest vector clock of the versions written by client $c$.}
    \Statex \red{$\hrvc$: Highest vector clock of the versions read by client $c$.}
    \Statex \red{$\cvc_c$: Client's vector clock}

    \Statex
    \Function{\readkey}{$k, l$}
      \State $p^{i}_{d} \gets \Call{partition}{k}$

      \If{$l = \mr$}
        \State $vc_r \gets \hrvc$
        \State $vc_w \gets 0$
      \ElsIf{$l = \ryw$}
        \State $vc_r \gets 0$
        \State $vc_w \gets \hwvc$
      \ElsIf{$l = \mryw$}
        \State $vc_r \gets \hrvc$
        \State $vc_w \gets \hwvc$
      \EndIf

      \State $\langle v, vc, css \rangle \gets \send \Call{\readrequest}{k, vc_r, vc_w}$ to $p^{i}_{d}$

      \For{$j = 1 \ldots D$}
  \State $\hrvc[j] \gets \max \set{\hrvc[j], css[j]}$ \label{line:hrv-update}
	\State $\cvc_{c}[j] \gets \max \set{\cvc_{c}[j], vc[j]}$
	\label{line:ts-get}
	\State \hfill\Comment{\blue{$\ts(\readkey) \gets \cvc_{c}$}}
      \EndFor
      \State \Return $v$
    \EndFunction

    \Statex
    \Function{\updatekey}{$k, v, l$}
      \State $p^{i}_{d} \gets \Call{partition}{k}$

      \If{$l = \mw$}
        \State $cvc \gets \cvc_c^w$
      \ElsIf{$l = \wfr$}
        \State $cvc \gets \cvc_c^r$
      \ElsIf{$l = \mwfr$}
        \For{$i = 1 \ldots D$}
	       \State $cvc[i] \gets \max \set{\cvc_{c}^w[i], \cvc_{c}[i]}$
        \EndFor
      \EndIf

      \State $t \gets \send \Call{\updaterequest}{k, v, cvc}$ to $p^{i}_{d}$
      \State $\cvc_{c}[d] \gets t$
      \label{line:ts-put}
      \State $\hwvc[d] \gets t$
      \label{line:hwv-update}
      \Comment{\blue{$\ts(\updatekey) \gets \cvc_{c}^w$}}
      \State \Return \ok
    \EndFunction
  \end{algorithmic}
\end{algorithm}


==> figs/load.tex <==
% load.tex

\begin{figure}[h]
  \centering
  \subfigure[Latency]{
    \begin{minipage}[h]{0.46\linewidth}
      \centering
      \includegraphics[width = 1.0\textwidth]{figs/thread-latency}\label{fig:thread-latency}
    \end{minipage}
  }
  \subfigure[Throughput]{
    \begin{minipage}[h]{0.46\linewidth}
      \centering
      \includegraphics[width = 1.0\textwidth]{figs/thread-throughput}\label{fig:thread-throughput}
    \end{minipage}
  }
  \caption{The effect of load on the latency and throughput with 100\% local traffic}
  \label{fig:load}
\end{figure}


==> figs/ratio.tex <==
% ratio.tex

\begin{figure}[h]
  \centering
  \subfigure[Latency]{
    \begin{minipage}[h]{0.46\linewidth}
      \centering
      \includegraphics[width = 1.0\textwidth]{figs/rw-latency}\label{fig:ratio-latency}
    \end{minipage}
  }
  \subfigure[Throughput]{
    \begin{minipage}[h]{0.46\linewidth}
      \centering
      \includegraphics[width = 1.0\textwidth]{figs/rw-throughput}\label{fig:ratio-throughput}
    \end{minipage}
  }
  \caption{The effect of read/write ratio on the latency and throughput with 100\% local traffic}
  \label{fig:ratio}
\end{figure}



==> figs/remote-load.tex <==
% remote-load.tex

\begin{figure}[t]
  \centering
  \subfigure[Latency]{
    \begin{minipage}[h]{0.46\linewidth}
      \centering
      \includegraphics[width = 1.0\textwidth]{figs/remote-thread-latency}\label{fig:remote-thread-latency}
    \end{minipage}
  }
  \subfigure[Throughput]{
    \begin{minipage}[h]{0.46\linewidth}
      \centering
      \includegraphics[width = 1.0\textwidth]{figs/remote-thread-throughput}\label{fig:remote-thread-throughput}
    \end{minipage}
  }
  \caption{The effect of load on the latency and throughput with 25\% remote traffic}
  \label{fig:remote-load}
\end{figure}


==> figs/remote-ratio.tex <==
% remote-ratio.tex

\begin{figure}[h]
  \centering
  \subfigure[Latency]{
    \begin{minipage}[h]{0.46\linewidth}
      \centering
      \includegraphics[width = 1.0\textwidth]{figs/remote-rw-latency}\label{fig:remote-ratio-latency}
    \end{minipage}
  }
  \subfigure[Throughput]{
    \begin{minipage}[h]{0.46\linewidth}
      \centering
      \includegraphics[width = 1.0\textwidth]{figs/remote-rw-throughput}\label{fig:remote-ratio-throughput}
    \end{minipage}
  }
  \caption{The effect of read/write ratio on the latency and throughput with 25\% remote traffic}
  \label{fig:remote-ratio}
\end{figure}



==> sections/cc.tex <==
% cc.tex

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Causal Consistency vs. Session Guarantees}

We aim to show that

\begin{theorem}
  \begin{align*}
    \cc \triangleq & \ryw \land \mr \land \\
                   & \mwv \land \mwa \land \\
                   & \wfrv \land \wfra.
  \end{align*}
  where, $\cc$ is defined as follows in~\cite{PoEC:NOW2014}
  \begin{align*}
    \cc \triangleq &\retval(\mathcal{F}) \land \\
                   &\cv \land \\
                   &\ca \land \\
                   &\ev.
  \end{align*}
  and session guarantees are defined as follows in~\cite{RDT:POPL2014}
  \begin{align*}
    \ryw & \triangleq \so \subseteq \vis \\
    \mr  & \triangleq (\vis;\so) \subseteq \vis \\
    \mwv & \triangleq (\so;\vis) \subseteq \vis \\
    \mwa & \triangleq \so \subseteq \ar \\
    \wfrv & \triangleq (\vis;\so;\vis) \subseteq \vis\\
    \wfra & \triangleq (\vis;\so) \subseteq \ar
  \end{align*}
\end{theorem}

\begin{lemma}
  \[
    \cv \triangleq \ryw \land \mr \land \mwv \land \wfrv.
  \]
\end{lemma}

\begin{proof}
Let $A = ((E, \op, \rval, \so), \vis, \ar)$ be an abstract execution.
Let
\begin{align*}
  r_1 &= \so \cup (\vis;\so) \cup (\so;\vis) \cup (\vis;\so;\vis);\\
  r_2 &= (\vis \cup \so)^{+}.
\end{align*}
\begin{itemize}
  \item $r_2 \subseteq \vis \Rightarrow r_1 \subseteq \vis$.
    We have $r_1 \subseteq r_2$, so $r_1 \subseteq \vis$.
  \item $r_1 \subseteq \vis \Rightarrow r_2 \subseteq \vis$.
    We assume that two events $e,e' \in E$ such that $e \rel{r_2} e'$,
    we need to show that $e \rel{\vis} e'$.
    \begin{itemize}
      \item Case I: $e \rel{\so} e'$.
        Since $\so \subseteq r_1$, $e \rel{r_1} e'$.
        Due to $r_1 \subseteq \vis$, $e \rel{\vis} e'$.
      \item Case II: $e$ and $e'$ are events performed on different clients.
        There exists events $o$ (it may be $e$ itself) $o'$ (it may be $e'$ itself) such that $e \rel{\so} o \rel{\vis} o' \rel{\so} e'$.
        Since $r_1 \subseteq \vis$ and $(\so;\vis)\subseteq r_1$, $e\rel{\vis}o'\rel{\so}e'$.
        Then we have $e\rel{vis}e'$
    \end{itemize}
\end{itemize}
\end{proof}

\begin{lemma}
  \[
    \ca \triangleq \mwa \land \wfra.
  \]
\end{lemma}

\begin{proof}
Let $A = ((E, \op, \rval, \so), \vis, \ar)$ be an abstract execution.
Let
\begin{align*}
  r_1 &= \so \cup (\vis;\so);\\
  r_2 &= (\vis \cup \so)^{+}.
\end{align*}
\begin{itemize}
  \item $r_2 \subseteq \ar \Rightarrow r_1 \subseteq \ar$.
    We have $r_1 \subseteq r_2$, so $r_1 \subseteq \ar$.
  \item $r_1 \subseteq \ar \Rightarrow r_2 \subseteq \ar$.
    We assume that two events $e,e' \in E$ such that $e \rel{r_2} e'$,
    we need to show that $e \rel{\ar} e'$.
    \begin{itemize}
      \item Case I: $e \rel{\so} e'$.
        Since $\so \subseteq r_1$, $e \rel{r_1} e'$.
        Due to $r_1 \subseteq \ar$, $e \rel{\ar} e'$.
      \item Case II: $e$ and $e'$ are events performed on different clients.
        There exists events $o$ (it may be $e$ itself) $o'$ (it may be $e'$ itself) such that $e \rel{\so} o \rel{\vis} o' \rel{\so} e'$.
        Since $r_1 \subseteq \ar$ and $\so \cup (\vis;\so)\subseteq r_1$, $e\rel{\ar}o'\rel{\ar}e'$.
        Due to \ar{} is transitive, we have $e\rel{\ar}e'$.
    \end{itemize}
\end{itemize}
\end{proof}

我们证明了$\cv$和$\ca$和\cite{RDT:POPL2014}中的六个session guarantees之间的关系。这几个session guarantees的规约并未涉及在解释某个特定事件$e$ 的返回值时，对$e$的可见事件的部分或所有返回值需要被考虑的情况。因此猜想仅有这些session guarantees的规约并不能直接刻画某个特定的因果一致性的变体。例如，所有session guarantees的conjunction不和\cc{}(\wccv)等价。图\ref{fig:exp-wccv}和图\ref{fig:exp-not-wcc-wccv}中的执行分别满足和不满足\wccv{}。但是这两个执行都满足上述的所有session guarantees。

\begin{figure}[t]
  \centering
  \includegraphics[width = 0.35\textwidth]{figs/exp-wcc-not-cc-not-wccv}
  \caption{\wcc, but not \wccv}\label{fig:exp-not-wcc-wccv}
\end{figure}

\begin{figure}[t]
  \centering
  \includegraphics[width = 0.35\textwidth]{figs/exp-cc-wccv-not-scc-not-sc}
  \caption{\wccv}\label{fig:exp-wccv}
\end{figure}

所有session guarantees的conjunction也不和\wcc{}等价。图\ref{fig:exp-not-wcc-wccv}和图\ref{fig:exp-not-wcc}中的执行分别满足和不满足\wcc{}。但是这两个执行都满足上述的所有session guarantees。

\begin{figure}[t]
  \centering
  \includegraphics[width = 0.45\textwidth]{figs/exp-not-wcc}
  \caption{Not \wcc}\label{fig:exp-not-wcc}
\end{figure}


==> sections/curelc-comment.tex <==
% curelc-comment.tex

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\chapter{Cure}

The following is the Cure protocol~\cite{Cure:ICDCS2016} instrumented with Lamport clocks~\cite{Lamport:CACM1978} for each key.

\input{algs/cure-client}
\input{algs/cure-server}
\input{algs/cure-clock}
%%%%%%%%%%%%%%%%%%%%
\section{Algorithm~\ref{alg:client}: Client}
\label{section:alg-client}

Same as \cure.
%%%%%%%%%%%%%%%%%%%%
\section{Algorithm~\ref{alg:server}: Server}
\label{section:alg-server}

\begin{itemize}
  \item Adding Lamport clock $\lc^{m}_{d}[k]$ for key $k$
\end{itemize}

\begin{itemize}
  \item \manuel Line~\ref{line:get-css-max} of Algorithm~\ref{alg:server}. \\
  You update $\css[d]$ with the clients clock ($cvc[d]$),
  where $d$ is the id for the local data center. 
  I think this may be wrong as client's updates 
  may not be stable yet 
  (as there is no wait when a client issues an update).
  
  \hfwei Strictly speaking, it is wrong to update $\css^{m}_{d}[d]$ with $cvc[d]$. 
  However, the entry $\css^{m}_{d}[d]$ is not used in this protocol. 
  In particular, we have ``$vc[i] \le \css^{m}_{d}[i]$ 
  for \red{$i \neq d$}'' in the read rule 
  on Line~\ref{line:get-from}.
  
  I removed ``$i \neq d$'' from Line~\ref{line:get-no-d}
  just to make the code a little bit shorter, 
  which, however, makes it confusing.
  So I put it back; see Lines~\ref{line:get-no-d} and \ref{line:put-no-d} of Algorithm~\ref{alg:server} and
  Line~\ref{line:updatecss-no-d} of Algorithm~\ref{alg:clock}.
\end{itemize}
%%%%%%%%%%%%%%%%%%%%
\section{Algorithm~\ref{alg:clock}: Clock}
\label{section:alg-clock}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

==> sections/operational-proof.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Correctness Proof}

In this section, we prove the correctness of the protocol above.
We first define three sets of \pput{} events.
We define $\cwrites(c,t)$ to be
the set of all \pput{} events
done by client $c$ at time $t$.
Similarly, we define $\creads(c,t)$ to be
the set of all \pput{} events that
have written a value for some key
read by client $c$ at time $t$.
We also define $\swrites(s,t)$ to be
the set of all stable \pput{} events
known to $s$ in the local datacenter
when $c$'s request is applied at $s$ at time $t$.
Now we use the definitions above to
describe four session guarantees
defined in Section~\ref{section:tcc}.

Read your writes (\ryw): Let $g$ be a read by client $c$ at time $t$.
Event $g$ satisfies \ryw{}
if any $p\in \cwrites(c,t)$ is included in $\swrites(s,t')$
, where time $t'$ is when $g$ is applied at partition $s$.

Monotonic read (\mr): Let $g$ be a read by client $c$ at time $t$.
Event $g$ satisfies \mr{}
if any $p\in \creads(c,t)$ is included in $\swrites(s,t')$
, where time $t'$ is when $g$ is applied at partition $s$.

Monotonic write (\mw): Let $p$ be a write by client $c$ at time $t$.
Partition $s$ applies it at time $t'$.
Event $p$ satisfies \mw{}
if $p$ is included in $\swrites(s,t')$,
there is no \pput{} event $e$ ($e \neq p$) such that
$\cwrites(c,t)$ includes $e$
and $vc_p$ is smaller than $vc_e$.

Writes follow read (\wfr): Let $p$ be a write by client $c$ at time $t$.
Partition $s$ applies it at time $t'$.
Event $p$ satisfies \wfr{}
if $p$ is included in $\swrites(s,t')$,
there is no \pput{} event $e$ ($e \neq p$) such that
$\creads(c,t)$ includes $e$
and $vc_p$ is smaller than $vc_e$.

%Now we provide the correctness of the protocol provided in Section \ref{section:algorithm}.

%\begin{lemma} \label{lemma:stable-css}
%  Let $p_{d}^{m}$ be a partition,
%  and $p$ be a \pput{} event.
%  If $p$ has not been stable,
%  we have
%  \[
%      \exists i: \css_{d}^{m}[i] < vc_p[i].
%  \]
%\end{lemma}

%\begin{proof}
%  By Line~\ref{line:get-from} of Algorithm~\ref{alg:server}.
%\end{proof}

Now, we prove the correctness of the protocol
for session guarantees constraining \get{} events.

\begin{theorem}[$\mr$]  \label{thm:mr}
  Any \get{} event reading a key by client $c$
  at partition $p_{d}^{m}$ with $\hrvc$ satisfies $\mr$.
\end{theorem}

\begin{proof}
  Let $g$ be a \get{} event by client $c$
  reading the value of key $k$ at time $t$
  at partition $p_{d}^{m}$ and returns at time $t'$.
  Since $g$ returns at time $t'$, we have $\css_{d}^{m} \ge \hrvc$ at time $t'$
  according to Line~\ref{line:get-wait} of Algorithm~\ref{alg:server}.
  Suppose by a contradiction that
  $g$ does not satisfy $\mr$.
  This means that there exists a \pput{} event $e$ such that
  $e \in \creads(c,t)$ and $e \notin \swrites(p_{d}^{m},t')$.
  Since $e \notin \swrites(p_{d}^{m},t')$, there is some datacenter $i$ such that
  $\css_{d}^{m}[i] < vc_e[i]$ at time $t'$ according to Line~\ref{line:get-wait} of Algorithm~\ref{alg:server}.
  Since $e \in \creads(c,t)$, $\hrvc \ge vc_e$
  according to Line~\ref{line:hrv-update} of Algorithm~\ref{alg:client}
  and Line~\ref{line:get-from} of Algorithm~\ref{alg:server}.
  Thus, $\css_{d}^{m} \ge vc_e$ at time $t'$.
  Contradiction.
\end{proof}

We can prove the following theorem in a similar way.

\begin{theorem}[$\ryw$]  \label{thm:ryw}
  Any \get{} event reading a key by client $c$
  at partition $p_{d}^{m}$ with $\hwvc$ satisfies $\ryw$.
\end{theorem}

%\begin{proof}
%  Let $g$ be a \get{} event by client $c$
%  reading the value of key $k$ at time $t$
%  at partition $p_{d}^{m}$ and returns at time $t'$.
%  Since $g$ returns at time $t'$, we have $\css_{d}^{m} \ge \hwvc$
%  according to Line~\ref{line:get-wait} of Algorithm~\ref{alg:server}.
%  Suppose by a contradiction that
%  $g$ does not satisfy $\ryw$.
%  This means that there exists a \pput{} event $e$ such that
%  $e \in \cwrites(c,t)$ and $e \notin \swrites(p_{d}^{m},t')$.
%  Since $e \notin \swrites(p_{d}^{m},t')$ and $e$ is a local \pput{} in datacenter $d$,
%  $\css_{d}^{m}[d] < vc_e[d]$ at time $t'$.
%  Since $e \in \cwrites(c,t)$, $\hwvc \ge vc_e$
%  according to Line~\ref{line:hwv-update} of Algorithm~\ref{alg:client}.
%  Thus, $\css_{d}^{m}[d] \ge vc_e[d]$ at time $t'$.
%  Contradiction.
%\end{proof}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
Now, we prove the correctness of the protocol
for session guarantees constraining \pput{} events.

\begin{theorem}[$\mw$]  \label{thm:mw}
  Any \pput{} event writing a key by client $c$
  at partition $p_{d}^{m}$ with $\cvc_c^w$ satisfies $\mw$.
\end{theorem}

\begin{proof}
  Let $p$ be a \pput{} event by client $c$
  writing to key $k$ at time $t$
  at partition $p_{d}^{m}$ and returns at $t'$.
  Suppose by a contradiction that
  $p$ does not satisfy $\mw$.
  This means that there exists
  a \pput{} event $e$ ($e \neq p$) such that
  $e \in \cwrites(c,t)$ and $vc_p < vc_e$.
  We have $\cvc_c^{w} \ge vc_e$ at time $t$
  according to Line~\ref{line:ts-put} of Algorithm~\ref{alg:client}.
  By Line~\ref{line:wait-clock} and Line~\ref{line:put-d-clock} of Algorithm~\ref{alg:server},
  we have $vc_p > \cvc_c^w$ at time $t'$. Thus, $vc_p > vc_e$.
  Contradiction.
\end{proof}

We can prove the following theorem in a similar way.

\begin{theorem}[$\wfr$]  \label{thm:wfr}
  Any \pput{} event writing a key by client $c$
  at partition $p_{d}^{m}$ with $\cvc_c^r$ satisfies $\wfr$.
\end{theorem}

%\begin{proof}
%  Let $p$ be a \pput{} event $p$ by client $c$
%  writing the value $v$ for key $k$ at time $t$
%  to partition $p_{d}^{m}$ and returns at $t'$.
%  Suppose by a contradiction that
%  $p$ does not satisfy $\wfr$.
%  This means that there exists
%  event $e$ ($e \neq p$) such that
%  $e \in \creads(c,t)$ and $vc_p < vc_e$.
%  We have $\cvc_c^{r} > vc_e$ at time $t$
%  according to Line~\ref{line:ts-get} of Algorithm~\ref{alg:client}.
%  By Line~\ref{line:wait-clock} and Line~\ref{line:put-d-clock} of Algorithm~\ref{alg:server},
%  we have $vc_p > \cvc_c^r$ at time $t'$. Thus, $vc_p > vc_e$.
%  Contradiction.
%\end{proof}


==> sections/partition.tex <==
% partition.tex

\begin{figure*}[t]
  \centering
  \subfigure[Latency]{
    \begin{minipage}[t]{0.45\linewidth}
      \centering
      \includegraphics[width = 0.95\textwidth]{figs/partition-latency}
    \end{minipage}
  }
  \subfigure[Throughput]{
    \begin{minipage}[t]{0.45\linewidth}
      \centering
      \includegraphics[width=0.95\textwidth]{figs/partition-throughput}
    \end{minipage}
  }
  \caption{The effect of deployment on the latency and throughput}
  \label{fig:partition}
\end{figure*}


==> sections/proof-comment.tex <==
% proof-comment.tex

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\chapter{Correctness Proof}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Specification}  \label{section:spec}

We aim to show that
\begin{theorem}
  \[
    \cure \models \cc(\fkvs)
  \]
  where, $\cc$ is defined as follows in~\cite{PoEC:NOW2014}
  \begin{align*}
    \cc \triangleq &\retval(\fkvs) \land \\
                   &\cv \land \\
                   &\ca \land \\
                   &\ev.
  \end{align*}
\end{theorem}

We need to show that every history $H = (O, \so)$ of \cure{} satisfies $\cc$, by showing that
\[
  \exists\; \vis, \ar: A \triangleq (H, \vis, \ar) \models \cc
\]
where, $O$ is the set of operations in $H$.

We define $G$, $P$, $P_k$ to be the set of \readkey{} operations,
the set of \updatekey{} operations, and the set of \updatekey{} operations on key $k$, respectively.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Timestamps}  \label{section:ts}

Cure attaches a unique timestamp $\ts(e) = \cvc_{c}$ to each \updatekey{} operation $e$;
see Line~\ref{line:ts-put} of Algorithm~\ref{alg:client}.
Note that for \updatekey{} $e$, $\ts(e) = vc_{e}$
where $vc_{e}$ is the vector clock attached to $e$.
We also define $\ts$ for \readkey{} operations in a similar way;
see Line~\ref{line:ts-get} of Algorithm~\ref{alg:client}.
Each timestamp is a vector clock, one entry per DC.
We define a partial order over timestamps as follows:
\[
  \ts(e) \le \ts(f) \iff \forall d: \ts(e)[d] \le \ts(f)[d]
\]
\[
  \ts(e) < \ts(f) \iff (\forall d: \ts(e)[d] \le \ts(f)[d]) \land (\exists d: \ts(e)[d] < \ts(f)[d])
\]
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Visibility Relation}  \label{section:vis}

The visibility relation $\vis$ is derived from the following read-from order $\rf$.
\begin{definition}  \label{def:rf}
  $(e, f) \in \rf$ if and only if $e = \updatekey(k, v) \triangleright \langle k, v, vc \rangle$ 
  and $f = \readkey(k) \triangleright \langle v, vc \rangle$ for some key $k$.
\end{definition}

\begin{definition}  \label{def:vis}
  The visibility relation $\vis$ is defined to be the transitive closure of
  the union of session order \so{} and read-from order $\rf$.
  Formally, 
  \[
    \vis = (\so \cup \rf)^{+}.
  \]
\end{definition}

The following lemma asserts that the visibility order $\vis$ is reflected 
in $\ts$ and $\eo$ (the execution order).
\begin{lemma}  \label{lemma:vis-ts-eo}
  Let $o_1$ and $o_2$ be two operations of history $H$. We have
  \[
    o_1 \rel{\vis} o_2 \implies \ts(o_1) \le \ts(o_2).
  \]
  Furthermore, if $o_2$ is a \updatekey, we have
  \[
    o_1 \rel{\vis} o_2 \land o_2 \in P \implies \ts(o_1) < \ts(o_2).
  \]
  Additionally,
  \[
    o_1 \rel{\vis} o_2 \implies o_1^{\request} \rel{\eo} o_2^{\request}.
  \]
  Here, $o^{\request}$ represents the event of processing $o$ by some server.
\end{lemma}

\begin{proof}  \label{proof:vis-ts-eo}
  By induction on the structure of the visibility relation $\vis$.

  \begin{itemize}
    \item \textsc{Case I}: $o_1 \rel{so|_c} o_2$ for some client $c$.
      \begin{itemize}
    	\item $\cvc_{c}$ is monotonically increasing. So $\ts(o_1) \le \ts(o_2)$.
    	\item If $o_2$ is a \updatekey, $\cvc_{c}$ is increased 
    	  due to the waiting condition on Line~\ref{line:wait-clock} of Algorithm~\ref{alg:server}.
    	  So $\ts(o_1) < \ts(o_2)$.
    	\item Since each client $c$ in $H$ is well-formed, $o_1^{\request} \rel{\eo} o_2^{\request}$.
      \end{itemize}
    \item \textsc{Case II}: $o_1 \rel{\rf} o_2$.
      \begin{itemize}
        \item $\ts(o_1) \le \ts(o_2)$ holds due to Line~\ref{line:ts-get} of Algorithm~\ref{alg:client}.
    	\item $o_2$ is a \readkey{}.
    	\item Since $o_1$ can be read by $o_2$ on Line~\ref{line:get-from} of Algorithm~\ref{alg:server}
    	  only after it has been performed on Line~\ref{line:put} of Algorithm~\ref{alg:server}
    	  (no matter whether $o_1$ is a local or a remote \updatekey{} w.r.t $o_2$), 
    	  $o_1^{\request} \rel{\eo} o_2^{\request}$.
      \end{itemize}
    \item \textsc{Case III}: There is some operation $o$ such that $o_1 \rel{\vis} o \rel{\vis} o_2$.
      \begin{itemize}
    	\item By induction, we have $\ts(o_1) \le \ts(o) \le \ts(o_2)$.
    	\item By induction, if $o_2$ is a \updatekey, $\ts(o_1) \le \ts(o) < \ts(o_2)$.
    	\item By induction, we have $o_1^{\request} \rel{\eo} o^{\request} \rel{\eo} o_2^{\request}$.
      \end{itemize}
  \end{itemize}
\end{proof}

\begin{theorem} \label{thm:vis-partial}
  The visibility relation $\vis$ is a partial order.
\end{theorem}

\begin{proof}
  It suffices to show that $\rel{\vis}$ is acyclic.
  Suppose by contradiction that there is a cycle 
  $\mathcal{C}: o_1 \rel{\vis} o_2 \rel{\vis} \cdots \rel{\vis} o_i \rel{\vis} o_1$.
  By Lemma~\ref{lemma:vis-ts-eo}, 
  all the operations in $\mathcal{C}$ are \readkey{} operations
  and they have the same $\ts$.
  Furthermore, all of them cannot be in the same client,
  as this would imply a cycle in session order.
  Suppose $o$ and $o'$ in $\mathcal{C}$ are on different clients.
  Since $o \rel{\vis} o'$ and both operations are \readkey{} operations,
  there must be some \updatekey{} $o''$ such that $o \rel{\vis} o'' \rel{\vis} o'$.
  By Lemma~\ref{lemma:vis-ts-eo}, $\ts(o) < \ts(o'') \le \ts(o')$.
  Contradiction.
\end{proof}

The happens-before relation $\hb$ is the transitive closure of 
the union of session order and visibility~\cite{PoEC:NOW2014}.
\begin{definition}  \label{def:hb}
  \[
    \hb \triangleq (\so \cup \vis).
  \]
\end{definition}

The following theorem implies that $A \models \cv$.
\begin{theorem}  \label{thm:cv}
  \[
    \hb \subseteq \vis.
  \]
\end{theorem}

\begin{proof} \label{proof:cv}
  By definitions of $\hb$ and $\vis$, we have $\hb = \vis$.
\end{proof}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Arbitration Relation}  \label{section:ar}

\begin{definition}  \label{def:ark}
  The per-key ordering $\ar_k$ is the total order on $P_{k}$, 
  defined by their Lamport clocks with data center $d$ for tie-breaking.
\end{definition}

\begin{definition}  \label{def:ar}
  We define $\ar$ on all \updatekey{} operations as any linear extension of 
  $\vis \cup \bigcup\limits_{k} \ar_{k}$.
\end{definition}

The following lemma ensures that $\ar$ is well-defined, i.e., acyclic.
\begin{lemma}  \label{lemma:ar-acyclic}
  For each $k$, $\ar_k$ is consistent with $\vis$. 
  Formally,
  \[
    \forall e, f \in P_k: e \rel{\vis} f \implies e \rel{\ar_k} f.
  \]
\end{lemma}

\begin{proof}  \label{proof:ar-acyclic}
  This holds due to the properties of Lamport clocks.
\end{proof}

The following theorem implies that $A \models \ca$.
\begin{theorem}  \label{thm:ca}
  \[
    \hb \subseteq \ar.
  \]
\end{theorem}

\begin{proof}  \label{proof:thm:ca}
  By the definition of \hb{} and \ar{}.
\end{proof}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Return Values}  \label{section:rval}

We need to show that
\[
  A \models \retval(\fkvs).
\]

The key is to show that each \readkey{} operation $e \in G_{k}$ returns 
the correct value, denoted by $\rval(e)$, in Cure w.r.t the specification $\fkvs$:
\[
  \forall e \in G_{k}: \rval(e) = \fkvs(e, \vis^{-1}(e)|_{P_{k}}, \vis, \ar)
\]

Suppose that $e$ is issued by client $c$ to partition $p^{m}_{d}$.
We first show, in the following theorem, 
that at the time $e$ returns on partition $p^{m}_{d}$
(Line~\ref{line:get-from} of Algorithm~\ref{alg:server}),
the set $S$ of stabilized operations on $k$ in $\store^{m}_{d}$ of Cure
is a superset of the set $V$ of \updatekey{} operations on $k$ 
visible to $e$ in terms of $\vis$.
\begin{theorem}  \label{thm:visible-stable}
  \[
    \red{V} \triangleq \vis^{-1}(e)|_{P_{k}} \subseteq 
    \Big\{f \in P_{k} : f \triangleright \langle k, v_{f}, vc_{f} \rangle \in (\store^{m}_{d})_{e} \land vc_{f}[i] \le (\css^{m}_{d})_{e}[i] \text{ for } i \neq d \Big\}
    \triangleq \red{S}
  \]
  where, $(\store^{m}_{d})_{e}$ and $(\css^{m}_{d})_{e}$ are the values of
  $\store^{m}_{d}$ and $\css^{m}_{d}$ when $e$ is performed after 
  Line~\ref{line:get-from} of Algorithm~\ref{alg:server}.
  (We use similar notations for \updatekey{} operations below, in which case
  we refer to values after Line~\ref{line:put} of Algorithm~\ref{alg:server}.)
\end{theorem}

\begin{proof}  \label{proof:visible-stable}
  For each $g \triangleright \langle k, v_g, vc_g \rangle \in V$, 
  we need to show that $g \in S$, i.e.,
  $g \in (\store^{m}_{d})_{e}$ and $vc_{g}[i] \le (\css^{m}_{d})_{e}[i]$ 
  for $i \neq d$.
  We perform case analysis according to whether $g$ is a local update 
  w.r.t data center $d$ or a remote one.
  \begin{itemize}
    \item $g$ is a local update.
      \begin{itemize}
        \item Since $g \rel{\vis} e$, $g \rel{\eo} e$ by 
          Lemma~\ref{lemma:vis-ts-eo}, i.e., $g$ is performed before $e$. 
          Therefore, $g \in (\store^{m}_{d})_{e}$.
        \item According to Line~\ref{line:put-css-max} of 
          Algorithm~\ref{alg:server}, $vc_{g}[i] \le {(\css^{m}_{d})}_{g}[i]$ 
          for $i \neq d$.
          According to Line~\ref{line:get-css-max} of 
          Algorithm~\ref{alg:server}, 
          $(\css^{m}_{d})_{g}[i] \le (\css^{m}_{d})_{e}[i]$ for $i \neq d$. 
          Therefore, $vc_{g}[i] \le (\css^{m}_{d}[i])_{e}$ for $i \neq d$.
          
          \alexey I was confused about the case of ``$g$ is a local update''.
          But I don't understand the logic of relying on lines 3 and 8 of Algorithm 2.
          Note that the events $g$ and $e$ may be done by different clients (at the same partition and DC),
          so I don't see how the above lines help you.

          \hfwei First, according to Lines~\ref{line:put-d-clock} and \ref{line:put} of Algorithm~\ref{alg:server}, 
          $vc_{g}[i] = cvc[i]$ for $i \neq d$.
          Then, according to Line~\ref{line:put-css-max} of Algorithm~\ref{alg:server},
          $vc_{g}[i] = cvc[i] \le (\css^{m}_{d})_{g}[i]$ for $i \neq d$,
          since we have computed the $\max$.
          Finally, $(\css^{m}_{d})_{g}[i] \le (\css^{m}_{d})_{e}[i]$ for $i \neq d$,
          because $\css^{m}_{d}[i]$ ($i \neq d$) is non-decreasing in time
          according to Line~\ref{line:get-css-max} of Algorithm~\ref{alg:server} and $g$ is performed before $e$.
      \end{itemize}
      
      \alexey In Theorem 5, case ``$g$ is a local updat'' 
      you seem to be using the update of $\css$ for the entry $d$, which doesn't happen in Cure.
      
      \hfwei $\css^{m}_{d}[d]$ is not used here because of
      the condition $i \neq d$.
      See also my comment to Manuel in Section~\ref{section:alg-server}.
    \item $g$ is a remote update.
      \begin{itemize}
        \item Since $g \rel{\vis} e$, there must be a \updatekey{} $p$
          (which may be $g$ itself) and a \readkey{} $q$ issued by client $c$ 
          on partition, e.g., $p^{n}_{d}$ (which may be $e$ itself) such that
          (generally, $p$ and $q$ may not be on key $k$.)
          \[
            g \rel{\vis} p \rel{\rf} q \rel{\so|_{c}} e.
          \]
          Since $p \rel{\rf} q$, $vc_{p}[i] \le (\css^{n}_{d})_{q}[i]$ 
          for $i \neq d$.
          Since $g \rel{\vis} p$, $\ts(g) < \ts(p)$ by 
          Lemma~\ref{lemma:vis-ts-eo}, i.e., $vc_{g} < vc_{p}$.
          Therefore, $vc_{g}[i] \le (\css^{n}_{d})_{q}[i]$ for $i \neq d$.
          Thus, $g$ has been replicated in data center $d$ when $q$ is performed.
          That is, $g \in (\store^{m}_{d})_{q}$.
          Since $q \rel{\so|_{c}} e$, $g \in (\store^{m}_{d})_{e}$.
          
          \alexey Case ``$g$ is a remote update''. 
          What are $p$ and $q$? 
          Do they have to be operations at different DCs?
          
          \hfwei Since $g$ is a remote update,
          it is issued by a different client than $c$.
          Since $\vis = (\so \cup \rf)^{+}$ and $e$ is on client $c$, the relation $g \rel{\vis} e$ must be
          established via $\rf$ relation.
          It may be $g \rel{\rf} e$; in this case
          $p = g$ and $q = e$.
          Otherwise, we have the case
          $g \rel{\vis} p \rel{\rf} q \rel{\so|_{c}} e$.
          Note that the \readkey{} $q$ is on client $c$.
          We have no particular requirement on the \updatekey{} $q$.
          
          \alexey ``Thus, $g$ has been replicated in data center $d \ldots$'': 
          some more justification might be in order here.
          Perhaps you need a proposition stating that 
          everything from other covered by $\css$ has been replicated.
          
          \hfwei We have derived from $g \rel{\vis} e$ that
          $vc_{g}[i] \le (\css^{n}_{d})_{q}[i]$ for $i \neq d$.
          In particular, $vc_{g}[j] \le (\css^{n}_{d})_{q}[j]$
          where $j$ ($j \neq d$) is the data center $g$ is located
          and $vc_{g}[j]$ refers to $g$ in data center $j$.
          This means that $g$ has been replicated in $d$.
        \item Since $q \rel{\so|_{c}} e$, $\ts(q)[i] \le (\css^{m}_{d})_{e}[i]$
          for $i \neq d$ (Line~\ref{line:get-css-max} of Algorithm~\ref{alg:server}).
          In addition, $vc_{p}[i] \le \ts(q)[i]$ for $i \neq d$ 
          (Line~\ref{line:ts-get} of Algorithm~\ref{alg:client}).
          Therefore, $vc_{g}[i] \le vc_{p}[i] \le \ts(q)[i] \le (\css^{m}_{d})_{e}[i]$ for $i \neq d$.
        \end{itemize}
  \end{itemize}
\end{proof}

\begin{theorem}  \label{thm:retval}
  \[
    \forall e \in G_{k}: \rval(e) = \fkvs(e, \vis^{-1}(e)|_{P_{k}}, \vis, \ar)
  \]
\end{theorem}

\begin{proof}  \label{proof:retval}
  Suppose $e$ reads from $f$ in $S$.
  By definition of $\vis$, $f \in V$.
  $V$ and $S$ are totally ordered according to the same $ar_k$ order.
  Since $f$ is the latest one in $S$ and $V \subseteq S$ 
  (Theorem~\ref{thm:visible-stable}), $f$ is also the latest one in $V$.
  Thus, $e$ reads from $f$ in $V$.
\end{proof}

\alexey I can't follow the proof of Theorem 6. 
What is $V, S$?

\hfwei $V$ ($V$ for ``visible'') and $S$ ($S$ for ``stable'')
are the same sets used in the proof for Theorem~\ref{thm:visible-stable}, 
described in the text just before this theorem.
Now I put the definitions of $V$ and $S$ in Theorem~\ref{thm:visible-stable}.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Eventual Visibility}  \label{section:ev}

\begin{theorem}  \label{thm:ev}
  \[
    A \models \cv.
  \]
\end{theorem}

\begin{proof}  \label{proof:ev}
  This holds due to the mechanism of propagating updates and heartbeats
  in order of increasing update timestamps and clock values
  and the mechanism of global stabilization.
\end{proof}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

==> sections/proof.tex <==
% proof.tex

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Correctness Proof} \label{ss:proof}

We aim to show that
\begin{theorem}
  \[
    \tccure \models \tcc,
  \]
  where, $\tcc$ is defined in Definition~\ref{def:tcc}.
\end{theorem}

We need to show that for every history $H = (E,\op,\so)$ of \cure{} satisfies \tcc{}.

\subsection{Notations}

We use $E, G, P, E_k, G_k, P_k$ and $G_l$ to denote the set
of all events, the set of \get{} events, the set
of \pput{} operations, the set of events on key $k$,
the set of \get{} events on key $k$, the set of
\pput{} events on key $k$ in a history and the set of
\get{} events with consistency level $l$, respectively.

For a \pput{} event $e$ on key $k$, consistency level $l$ and value $v_e$,
we write $e \vartriangleright \langle k, v_e, l, vc_e \rangle$
to emphasize that it is associated
with a vector clock $vc_e$ on Line~\ref{line:put}of Algorithm~\ref{alg:server}.
Similarly, For a \get{} event $e$ on key $k$ and consistency level $l$.
we write $e \vartriangleright \langle k, v_e, l, vc_e \rangle$
to emphasize that it returns value $v_e$ with
a vector clock $vc_e$, denoted as $\vc(e)$
on Line~\ref{line:get-from} of Algorithm~\ref{alg:server}.
We also use $lc_e$ to denote the Lamport clock for $e$ instrumented
on Line~\ref{line:lc-put} of Algorithm~\ref{alg:server}.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Vector Clocks} \label{sss:vc}

We denote the usual partial order``less-than" and
non-strict partial order ``less-than-or-equal-to" over vector
clocks by ``$<$" and ``$\leq$", respectively.
We first present lemmas about
$\cvc_c^r$ and $\cvc_c^w$,
and for any client $c$.

\begin{lemma}\label{lemma:cvc}
  Both $\cvc_c^r$ and $\cvc_c^w$ are non-decreasing in terms of ``$\leq$" over vector clocks.
\end{lemma}

\begin{proof}
$\cvc_c^r$ and $\cvc_c^w$ are updated only on Line 15 and Line 28 of Algorithm~\ref{alg:client}, respectively.
  \begin{itemize}
    \item On Line 15 of Algorithm~\ref{alg:client}, we take the maximum of the old $\cvc_c^r$ and another vector clock ($vc$).
    \item On Line 28 of Algorithm~\ref{alg:client}, $t$ is greater than $\cvc_c^w[d]$
        due to the wait condition on Line~\ref{line:wait-clock} of Algorithm~\ref{alg:server}.
  \end{itemize}
\end{proof}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\subsection{Execution Order} \label{sss:eo}
%
%\begin{definition}
%  Event $e_1$ is executed before event $e_2$,
%  denoted $e_1 \rel{\eo} e_2$ if $e_1^{\request}$
%  is executed before (in real-time) $e_2^{\request}$,
%  where $e^{\request}$ refers to Line 3
%  and Line 10 of Algorithm 2 for read and update, respectively.
%\end{definition}
%
%\begin{lemma}\label{lemma:so-eo}
%  \[
%    \so \subseteq \eo.
%  \]
%\end{lemma}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Timestamps} \label{sss:timestamps}

We first define timestamp $\ts(e)$ for each event $e$ as follows.

\begin{definition}[Timestamps] \label{def:timestamps}
  For a \get{} event $e$ issued by client $c$, $\ts(e) = \cvc_{c}^r$,
  where $\cvc_{c}^r$ is the last time of reads by client $c$.
  %and $s$ is the identifier of the server processing $e$
%  on Line~\ref{line:ts-get} for \get{} of Algorithm~\ref{alg:client}.
  Similarly, for a \pput{} event $e$ issued by client $c$, $\ts(e) = \cvc_{c}^w$,
  where $\cvc_{c}^w$ is the last time of writes by client $c$,
  and $s$ is the identifier of the server processing $e$
  on Line~\ref{line:ts-put} for \pput{} of Algorithm~\ref{alg:client}.
\end{definition}

Timestamps are compared lexicographically (we assume a
total order over the set of identifiers of servers).
For convenience, we also lift ``<" and ``$\leq$"
over timestamps (i.e. vector clocks) to ``$\ts_<$" and ``$\ts_{\leq}$".
That is,
\begin{align*}
  e_1 \rel{\ts_<} e_2 &\iff \ts(e_1) < \ts(e_2)\\
  e_1 \rel{\ts_{\leq}} e_2 &\iff \ts(e_1) \leq \ts(e_2)
\end{align*}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Visibility and Arbitration} \label{sss:visibility}

\begin{definition}[Read-from Relation] \label{def:rf}
  $(e, f) \in \rf$ if and only if $e = \pput(k, v, \_) \triangleright \langle k, v, \_, vc \rangle$
  and $f = \get(k, \_) \triangleright \langle k, v, \_, vc \rangle$ for some key $k$.
\end{definition}

\begin{definition}[Visibility] \label{def:visibility}
We define $\vis_{\ryw}, \vis_{\mr}$ and $\vis$ as follows:
  \begin{itemize}
    \item $\vis_{\ryw}$ is defined as
     \[
        \forall e\in P, f\in G_{\ryw}. e\rel{\vis_{\ryw}}f \Longleftrightarrow \vc(e) \leq \svc(f).
     \]
    \item $\vis_{\mr}$ is defined as
     \[
        \forall e\in P, f\in G_{\mr}. e\rel{\vis_{\mr}}f \Longleftrightarrow \vc(e) \leq \svc(f).
     \]
     \item $\vis$ is defined as
     \[ \vis \triangleq \vis_{\ryw} \cup \vis_{\mr}.\]
  \end{itemize}
\end{definition}

\begin{lemma}\label{lemma:vis-partial}
  The visibility relation \vis{} is a partial order.
\end{lemma}

\begin{proof}
  Since $\so, \vis_{\ryw}, \vis_{\mr}$ are partial orders,
  \vis{} is also a partial order according to Definition~\ref{def:visibility}.
\end{proof}

\begin{definition}[Per-key Ordering]
  The per-key ordering $\ar_{k}$ is the total order on $P_k$, defined by their timestamps
  with data center $d$ for tie-breaking.
\end{definition}

\begin{definition}[Arbitration] \label{def:ar}
  We define \ar{} on all \pput{} events as any linear extension of
  $\bigcup\limits_{k} \ar_{k}$.
\end{definition}

\begin{lemma}  \label{lemma:ar-vis}
  For each $k$, $\ar_k$ is consistent with $\vis$.
  Formally,
  \[
    \forall e, f \in P_k: e \rel{\vis} f \implies e \rel{\ar_k} f.
  \]
\end{lemma}

\begin{proof}  \label{proof:ar-acyclic}
  According to Definition~\ref{def:visibility}, there is only one case
  when $e$ and $f$ are performed on the same session.
  According to Line~\ref{line:lc-put} of Algorithm~\ref{alg:server},
  $\lc_e < \lc_{f}$.
  Therefore, $e \rel{\ar_k}f$.
\end{proof}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Session Guarantees} \label{sss:seg}

We first define three sets of \pput{} operations.

\begin{definition} \label{def:client-writes}
  $\cwrites(c,k,t)$ is the set of all \pput{} operations
  done by client $c$ when $c$ writes for key $k$ at time $t$.
\end{definition}

\begin{definition} \label{def:client-reads}
  $\creads(c,k,t)$ is the set of all \pput{} operations that
  have written a value for some key
  when client $c$ reads of key $k$ at time $t$.
\end{definition}

\begin{definition} \label{def:stable-writes}
  $\swrites(s,k,t)$ is the set of all stable \pput{} operations
  on server $s$ at time $t$.
\end{definition}

\begin{lemma} \label{lemma:stable-css}
  Let $p_{d}^{m}$ be a partition,
  and $p$ be a \pput{} operation.
  If $p$ has not been stable on partition $p_{d}^{m}$,
  we have
  \[
      \exists i: \css_{d}^{m}[i] < vc_p[i].
  \]
\end{lemma}

\begin{proof}
  By Line~\ref{line:get-from} of Algorithm~\ref{alg:server}.
\end{proof}

\begin{lemma} \label{lemma:cwrites}
Let $e$ be a \get{} event reading of key $k$ at time $t$,
and $o$ be a \pput{} event of a history $H$ , we have
\[
  o\rel{\so}e \Rightarrow o\in \cwrites(c,k,t).
\]
\end{lemma}

\begin{proof}
  By the definition of $\cwrites(c,k,t)$ in Def.~\ref{def:client-writes}.
\end{proof}

\begin{lemma} \label{lemma:cwrites}
Let $e$ be a \get{} event reading of key $k$ at time $t$,
and $o$ be a \pput{} event of a history $H$ , we have
\[
  o\rel{\vis}e \Rightarrow o\in \creads(c,k,t).
\]
\end{lemma}

\begin{proof}
  By the definition of $\creads(c,k,t)$ in Def.~\ref{def:client-reads}.
\end{proof}

\begin{theorem}
Let $e$ be a \get{} event on client $c$.
If $vc_r=0$ and $vc_w=\hwvc_c$ for $e$, $e$ satisfies \ryw.
\end{theorem}

\begin{proof}
  Assume that $e$ reads the value of key $k$
  at time $t$ to partition $p_{d}^{m}$
  and returns at time $t'$.
  Since $e$ returns at time $t'$,
  we have $\css_{d}^{m} \ge \hwvc$ at $t'$
  according to Line~\ref{line:get-wait} of Algorithm~\ref{alg:server}.
  Suppose by a contradiction that
  $e$ does not satisfy $\ryw$.
  This means that there exists a \pput{} operation $o$ such that
  $o \rel{\so} e$ but not $o \rel{\vis_{\ryw}} e$.
%  We distinguish whether $o$ is executed on $p_{d}^{m}$.
%  \begin{itemize}\item Case I: $o$ is executed on $p_{d}^{m}$.
    Since $o$ is not visible to $e$, $\vc(o)[i] > \svc(e)[i]$
    at time $t'$ for some $i$ by Definition~\ref{def:visibility},
    i.e., $o \notin \swrites(p_{d}^{m},k,t')$.
    Thus, $\css_{d}^{m}[i] < vc_o[i]$ for some $i$
    at time $t'$ by Lemma~\ref{lemma:stable-css}.
    Since $o \in \cwrites(c,k,t)$, we have $\hwvc \ge \vc(o)$
    according to Line~\ref{line:hwv-update} of Algorithm~\ref{alg:client}.
    Further, $\css_{d}^{m} \ge \vc(o)$ at time $t'$.
    Contradiction.
%    \item Case II: $o$ is not executed on $p_{d}^{m'} (m\neq m')$.
%    Since $o \in \cwrites(c,k,t)$, we have $\hwvc \ge vc_o$
%    according to Line~\ref{line:hwv-update} of Algorithm~\ref{alg:client}.
%    Since $o$ is not visible to $e$, there is some data center $i$
%    such that $\vc(o)[i] > \svc(e)[i] (\css_{d}^{m}[i])$ by Definition~\ref{def:visibility},
%    i.e., $o \notin \swrites(p_{d}^{m},k,t')$.
%    Further, we have $o$ is not in $o$ is not stable on $p_{d}^{m'}$.
%    Thus, there is some data center $i$ such that
%    $\css_{d}^{m'}[i] < \vc(o)[i]$ at time $t'$ by Lemma~\ref{lemma:stable-css}.
%    We have $\vc(o) < \hwvc < \css_{d}^{m}$ at time $t'$. Contradiction.
%  \end{itemize}
\end{proof}

\begin{theorem}
Let $e$ be a \get{} event on client $c$.
If $vc_r=\hrvc$ and $vc_w=0$ for $e$, $e$ satisfies \mr.
\end{theorem}

\begin{proof}
  Assume that $e$ reads the value of key $k$
  at time $t$ to partition $p_{d}^{m}$
  and returns at time $t'$.
  Since $e$ returns at time $t'$, we have $\css_{d}^{m} \ge \hrvc$ at time $t'$
  according to Line~\ref{line:get-wait} of Algorithm~\ref{alg:server}.
  Suppose by a contradiction that
  $e$ does not satisfy $\mr$.
  This means that there exists a \pput{} event $e_1$
  and a \get{} event $e_2$ such that
  $e_1 \rel{\vis} e_2 \rel{\so} e$ but not $e_1 \rel{\vis_{\mr}} e$.
  We have $e_1 \in \creads(c,k,t)$.
%  We distinguish whether $e_1$ is executed on $p_{d}^{m}$.
%  \begin{itemize}
%    \item Case I: $e_1$ is executed on $p_{d}^{m}$.
    Since $e_1 \in \creads(c,k,t)$, $\hrvc \ge \vc(e_1)$
    according to Line~\ref{line:hrv-update} of Algorithm~\ref{alg:client}
    and Line~\ref{line:get-from} of Algorithm~\ref{alg:server}.
    Further, we have $\css_{d}^{m} \ge \hrvc \ge \vc(e_1)$ at time t'.
    Since $e_1$ is not visible to $e$,
    $\svc(e)[i](=\css_{d}^{m}[i]) < \vc(e_1)[i]$ for some $i$
    at time $t'$ by Definition~\ref{def:visibility}.
    Contradiction.
%    \item Case II: $e_1$ is not executed on $p_{d}^{m}$.
%    Since $e_1 \in \creads(c,k,t)$, $e_1$ is stable
%    and we have $vc_{e_1} \le \css_{d}^{m}$ since it is stable.
%    Since $e_1$ is not visible to $e$ when e is executed on $p_{d}^{m}$,
%    we have $vc_{e_1} > \css_{d}^{m}$.
%    Contradiction.
%  \end{itemize}
\end{proof}

\begin{theorem} \label{thm:mw}
  Let $e$ be a \pput{} event on client $c$.
  If $dvc = \cvc_c^w$ for $e$, $e$ satisfies $\mw$.
\end{theorem}

\begin{proof}
  Assume that $e$ writes the value of key $k$
  at time $t$ to partition $p_{d}^{m}$
  and returns at time $t'$.
  Suppose by a contradiction that
  $e$ does not satisfy $\mw$.
  This means that there exists a \pput{} event $o$ such that
  $o \rel{\so} e$ but not $o \rel{\ar_{\mw}} e$.
  We have $\ts(o) < \ts(e)$ by Lemma~\ref{lemma:cvc}.
  $e$ can not be placed after $o$ according to Definition~\ref{def:ar}.
\end{proof}

\begin{theorem} \label{thm:mw}
  Let $e$ be a \pput{} event on client $c$.
  If $dvc = \cvc_c^r$ for $e$, $e$ satisfies $\wfr$.
\end{theorem}

\begin{proof}
  Assume that $e$ writes the value of key $k$
  at time $t$ to partition $p_{d}^{m}$
  and returns at time $t'$.
  Suppose by a contradiction that
  $e$ does not satisfy $\wfr$.
  This means that there exists a \pput{} event $e_1$
  and a \get{} event $e_2$ such that
  $e_1\rel{\vis}e_2\rel{\so}e$ but $e\rel{\ar_{\wfr}}e_1$.
  We have $\ts(e) < \ts(e_1)$ according to Definition~\ref{def:ar}.
  Since $e_1\rel{\vis}e_2$, $\ts(e_2) > \ts(e_1)$
  according to Line~\ref{line:cvcr-update} of Algorithm~\ref{alg:client}.
  We have $\ts(e) > \cvc_r$ according to the waiting condition
  on Line~\ref{line:wait-clock} of Algorithm~\ref{alg:server}.
  So we have $\ts(e) > \ts(e_1)$.
  Contradiction.
\end{proof}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Return Values} \label{sss:values}

We need to prove that $(H, \vis, \ar) \models \retval(\kvs)$.
The key is to show, for each \get{} event $e$, that
\[
  \forall e \in G: \rval(e) \in \eval_{\kvs}(\ctxt_{A}^{lv}(e), \op(e)),
\]
where $\ctxt_{A}^{lv}(e) = A|_{\vis_{lv}^{-1}(e), \op, \vis, \ar}$.
We only to construct a valid serialization for $e$, denoted $S_e$,
consisting of all \pput{} events in $\vis_{lv}^{-1}(e)$.
We denote the set of events in $S_e$ by $cP$,
namely, $cP \triangleq \vis_{lv}^{-1}(e) \cap P$.

\begin{theorem} \label{thm:mw}
  $S_{e}$ is a valid serialization of $cP$ when consistency level of $e$ is $\ryw$.
\end{theorem}

\begin{proof}
  Let $S_{\preceq e} \triangleq S_{e} \circ \langle e \rangle$,
  where `$\circ$' denotes concatenation.
  We need to show that each $\get(k)$ event in $S_{\preceq e}$
  returns the value written by the most recently preceding $\pput$ event on key $k$.
  Consider $g = \get(k)$ on client $c$ in $S_{\preceq e}$.
  Suppose $p \rel{\rf} g$ and $p$ is on client $i$.
  We must show that no other $\pput(k, \_, \_)$ events place in between $p$ and $g$ in $S_{\preceq e}$.
  Suppose by contradiction that event $p' = \pput(k, \_, \_)$ on client $j$ does.
  We distinguish between $j = c$ and $j \neq c$.
  \begin{itemize}
    \item Case I: $j=c$.
      Since $p \rel{\ar} p'$, $\ts(p) < \ts(p')$.
      Since $j = c$, $p' \rel{\so} g$.
      When $g$ is requested by client $c$, $\hwvc \ge \ts(p') > \ts(p)$.
      It is impossible for $g$ to read from $p$
      on Line~\ref{line:get-from} of Algorithm~\ref{alg:server}.
    \item Case II: $j \neq c$.

  \end{itemize}
\end{proof}


==> sections/temp.tex <==

%\begin{definition} \label{def:client-writes}
%  $\cwrites(c,k,t)$ is the set of all \pput{} operations
%  done by client $c$ when $c$ writes for key $k$ at time $t$.
%\end{definition}
%
%\begin{definition} \label{def:client-reads}
%  $\creads(c,k,t)$ is the set of all \pput{} operations that
%  have written a value for some key
%  when client $c$ reads of key $k$ at time $t$.
%\end{definition}
%
%\begin{definition} \label{def:stable-writes}
%  $\swrites(s,k,t)$ is the set of all stable \pput{} operations
%  on server $s$ when the request for key $k$ is executed at time $t$.
%\end{definition}

%\begin{definition}[\it{read-your-writes}] \label{def:cross-key-ryw}
%  Let $g$ be an operation by client $c$ that
%  reads the value of key $k$ at time $t$ at server $s$.
%  Operation $o$ satisfies read-your-writes consistency
%  if any $p\in \cwrites(c,k,t)$ is included in $\swrites(s,k,t')$
%  where $t'$ is the time when server s reads value for key $k$.
%\end{definition}
%
%\begin{definition}[\it{monotonic-read}] \label{def:cross-key-mr}
%  Let $g$ be an operation by client $c$ that
%  reads the value of key $k$ at time $t$ at server $s$.
%  Operation $o$ satisfies monotonic-read consistency
%  if any $p\in \creads(c,k,t)$ is included in $\swrites(s,k,t')$
%  where $t'$ is the time when server s reads value for key $k$.
%\end{definition}
%
%\begin{definition}[\it{monotonic-write}] \label{def:cross-key-mw}
%  Let $p$ be an operation by client $c$ that
%  writes a value for key $k$ at time $t$ at server $s$.
%  Operation $o$ satisfies monotonic-write consistency
%  if $p$ is included in $\swrites(s,k,t')$ at any time $t'$
%  no client accessing $s$ reads a value written by a \pput{} operation $o$ such that
%  $o \neq p$ and $\cwrites(c,k,t)$ includes $o$.
%\end{definition}
%
%\begin{definition}[\it{write-follows-reads}] \label{def:per-key-wfr}
%  Let $p$ be an operation by client $c$ that
%  writes a value for key $k$ at time $t$ at server $s$.
%  Operation $o$ satisfies write-follows-reads consistency
%  if $p$ is included in $\swrites(s,k,t')$ at any time $t'$
%  no client accessing $s$ reads a value written by a \pput{} operation $o$ such that
%  $o \neq p$ and $\creads(c,k,t)$ includes $o$.
%\end{definition}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\subsection{Session Guarantees} \label{section:sg}

==> tables/cases.tex <==
% cases.tex

\begin{table}[t]
  \centering
  \caption{Legend for Figure~\ref{fig:ratio} and ~\ref{fig:load}}
  \label{table:cases}
  \renewcommand{\arraystretch}{1.1}
  \begin{tabular}{l|l|l}
    \hline
    Legend & Read Guarantee & Write Guarantee \\
    \hline \hline
    $\ec/\ec$ & eventual consistency & eventual consistency \\
    \hline
    $\cc/\cc$ & causal consistency & causal consistency \\
    \hline
    $\ryw/\mw$ & read your writes & monotonic write \\
    \hline
    $\ryw/\wfr$ & Read Your Writes & writes follow reads \\
    \hline
    $\mr/\mw$ & monotonic read & monotonic write \\
    \hline
    $\mr/\wfr$ & monotonic read & writes follow reads \\
    \hline
%    $\ec/\mw$ & eventual consistency & monotonic write \\
%    \hline
%    $\ryw/\ec$ & read your writes & eventual consistency \\
  \end{tabular}
\end{table}


==> tables/table-session-guarantees.tex <==
% table-consistency-models.tex

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{table*}[!h]
  \caption{Session guarantees specified in the $(vis, ar, V)$ specification framework.
    (New variants are marked with $[\ast]$.)}
  \label{tbl:session-guarantees}
  \centering
  \resizebox{0.80\textwidth}{!}{
  \renewcommand{\arraystretch}{1.5}
  \begin{tabular}{c|c|c|c|c|c}
    \hline
    \multicolumn{2}{c|}{Consistency Levels}
    & Alternative Names
    & $\vis$
    & $\ar$
    & $V(e)$
    \\ \hline
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
    \multirow{6}{*}{\tabincell{c}{Session \\ Guarantees}}
    &\ryw{} (Def. 3.1~\cite{SESSION:PDIS1994})
    & \tabincell{c}{\textsc{ReadMyWrites} (Def. 5.1.1~\cite{PoEC:NOW2014})\\
                    \textsc{ReadYourWrites} (Def. 23~\cite{Consistency:CSUR2016})}
    & $\so \subseteq \vis$
    & -%ar
    & $V(e) = \emptyset$
    \\ \cline{2-6}
    &\mr{} (Def. 3.2~\cite{SESSION:PDIS1994})
    & \textsc{MonotonicReads} (Def. 22~\cite{Consistency:CSUR2016})
    & $(\vis;\so) \subseteq \vis$
    & -%ar
    & $V(e) = \so^{-1}(e)$
    \\ \cline{2-6}
    & \mw{} (Def. 3.4~\cite{SESSION:PDIS1994})
    & \textsc{MonotonicWrites} (Def. 24~\cite{Consistency:CSUR2016})
    & \multirow{2}{*}{$(\so;\vis) \subseteq \vis$}
    & $\so \subseteq \ar$
    & \multirow{2}{*}{$V(e) = \emptyset$}
    \\ \cline{2-3} \cline{5-5}
    & \mwc
    & [$\ast$]
    & %vis
    & $\so \subseteq \ar \land \tord{\ar, E}$
    & %V
    \\ \cline{2-6}
    & \wfr{} (Def. 3.3~\cite{SESSION:PDIS1994})
    & \textsc{WriteFollwsReads} (Def. 25~\cite{Consistency:CSUR2016})
    & \multirow{2}{*}{$(\vis;\so;\vis) \subseteq \vis$}
    & $(\vis;\so) \subseteq \ar$
    & \multirow{2}{*}{$V(e) = \vis^{-1}(e)$}
    \\ \cline{2-3} \cline{5-5}
    & \wfrc
    & [$\ast$]
    & %vis
    & $(\vis;\so) \subseteq \ar \land \tord{\ar, E}$
    & %V
    \\ \hline
  \end{tabular}}
\end{table*}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

